Gauge-Invariant Energy Functional in Relativistic Schroedinger Theory

The non-invariant energy functional of the preceding paper is improved in order to obtain its gauge-invariant form by strictly taking into account the non-Abelian character of Relativistic Schroedinger Theory (RST). As an application of the results, the dichotomy of positronium with respect to singlet and triplet states is discussed (ortho- and para-positronium). The degeneracy of the ortho- and para-states occurs in RST if (i) the magnetic interactions are neglected (as in the conventional theory) and (ii) the anisotropy of the electric interaction potential is disregarded. In view of such a very crude approximation procedure, the non-relativistic positronium spectrum in RST agrees amazingly well with the conventional predictions.

==> abstr_kurz.tex <==
\title{\bf Gauge-Invariant Energy Functional\\ in\\ Relativistic Schr\"odinger Theory}
\author{M.\ Mattes and M.\ Sorg} %\\[1cm] II.\ Institut f\"ur Theoretische Physik der Universit\"at Stuttgart\\ Pfaffenwaldring 57 \\ D 70550 Stuttgart, Germany
\date{ }
\maketitle
\begin{abstract}
  The \emph{non-invariant} energy functional of the preceding paper is improved in order
  to obtain its \emph{gauge-invariant} form by strictly taking into account the
  non-Abelian character of Relativistic Schr\"odinger Theory (RST). As an application of
  the results, the dichotomy of positronium with respect to singlet and triplet states is
  discussed (ortho- and para-positronium). The \emph{degeneracy} of the ortho- and
  para-states occurs in RST if \textbf{(i)} the magnetic interactions are neglected (as in
  the conventional theory) and \textbf{(ii)} the anisotropy of the electric interaction
  potential is disregarded. In view of such a very crude approximation procedure, the
  non-relativistic positronium spectrum in RST agrees amazingly well with the conventional
  predictions. 

  \vspace{2.5cm}
  \noindent
 \textsc{PACS Numbers:  03.65.Pm - Relativistic
  Wave Equations; 03.65.Ge - Solutions of Wave Equations: Bound States; 03.65.Sq -
  Semiclassical Theories and Applications; 03.75.b - Matter Waves}

  \clearpage
  \phantom{a}
\end{abstract}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> einl_kap6.tex <==
Once the emergence of the ortho/para dichotomy has been clarified in RST, there naturally
arises the question of degeneracy of the corresponding singlet and triplet states. But
here it should be clear that, corresponding to the present state of the art, this question
can be discussed only from a rather qualitative point of view because exact (analytic or
numerical) solutions of the RST two-particle eigenvalue problem are presently not
known. Nevertheless, the knowledge of the exact form of the RST energy functional~$\ETT$
(\ref{eq:IV.20}) admits to draw same general conclusions concerning this question of
degeneracy.

First, it will be necessary to define some level of approximation which corresponds to the
conventional situation (\ref{eq:V.13}), where the singlet and triplet states carry the
same energy. As a matter of course, this first approximation step will be essentially the
same in RST as in the conventional theory, namely the neglection of the magnetic
interactions ($\leadsto$ \emph{``electrostatic approximation''}). This neglection of the
magnetic forces, however, does not yet entail the mathematical equivalence of the
eigenvalue equations for the ortho- and para- configurations, indeed there persists a
crucial kinematical difference: whereas the current of the singlet states ($\leadsto$
\emph{``para-current''}~$\vec{k}_p$) must always encircle the axis of rotational symmetry
(i.e.\ the z-axis) and thus realizes a cylindrical structure, the
\emph{``ortho-current''}~$\vec{k}_b$ can own this cylindrical geometry only for
non-vanishing angular momentum~$(j_z=\pm 1)$, but for vanishing angular momentum~$j_z$ it
is required to undergo a \emph{toroidal} geometry (previously discussed in
ref.~\cite{x}). In the present paper, we restrict ourselves to the cylindrical structures
(i.e.~$j_z=0$ for the singlet states and~$j_z=-1$ for the triplet states), but even within
this subclass of the cylindrical configurations the link between the charge
densities~$\bpko$ and the wave amplitudes~$\bpMRpm,\bpMSpm$ looks different: for the
para-configurations, the essential angular variability of~$\pko(r)$ goes
like~$(\sin\vartheta)^{-1}$, cf.\ (\ref{eq:VI.17}); but for the ortho-densities~$\bkn$
there occurs a certain subdichotomy, see figure ?, in such a way that both forms of
ortho-matter with density~$\bkn$ are pressed off the rotational axis upon which they
become zero~$({}^{(b)}k_0 \big|_{\vartheta=0,\pi}=0)$.

Clearly, this specific distribution of ortho- and para-matter is responsible for the
difference in angular momentum (i.e.~$j_z=0$ for the para-distribution being concentrated
close to the rotational axis~$(\sim(\sin\vartheta)^{-1})$ and~$j_z=-1$ for the
ortho-distribution concentrated off the z-axis~$(\sim \sin\vartheta)$). However such a
redistribution of the charge densities does imply also a corresponding alteration of the
electrostatic interaction energy~$\eER$ so that the ortho- and para-configuration would
always carry different energy~$\ET$ and the ortho/para degeneracy would be spoiled. Thus
one is forced to conclude that, in order to encounter the degeneracy phenomenon in RST, it
is not sufficient to neglect the magnetic interactions as is the case with the
conventional.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> inhalt_uebergross_dina4.tex <==
\begin{center}
  {\Large\textbf{Contents}}
\end{center}

\begin{itemize}
\item[I] \textbf{Introduction and Survey of Results\dotfill 5}
\item[II] \textbf{Relativistic Schr\"odinger Theory\dotfill 14}
  \begin{itemize}
  \item[1.] \emph{Matter Fields \dotfill 14}
  \item[2.] \emph{Gauge Fields \dotfill 16}
  \end{itemize}
 \item[III] \textbf{Gauge Invariance and Entanglement \dotfill 19}
   \begin{itemize}
   \item[1.] \emph{Gauge Structure \dotfill 20}
   \item[2.] \emph{Mass Eigenvalue Equations \dotfill 23}
   \item[3.] \emph{Gauge Field Equations\dotfill 24}
   \item[4.] \emph{Linearization and Gauge Invariance \dotfill 26}
   \item[5.] \emph{RST Entanglement \dotfill 27}
   \item[6.] \emph{Boundary Conditions and Entanglement Charge \dotfill 30}   
   \end{itemize}
 \item[IV] \textbf{Gauge-Invariant Energy Functional \dotfill 34}
   \begin{itemize}
   \item[1.] \emph{Generalized Poisson Identities \dotfill 34}
   \item[2.] \emph{Exchange Identities \dotfill 36}
   \item[3.] \emph{Relativistic Energy Functional \dotfill 37}
   \item[4.] \emph{Non-Relativistic Variational Principle\dotfill 40}
     \begin{itemize}
     \item[] \emph{Non-Relativistic Eigenvalue Equations \dotfill 41}
     \item[] \emph{Non-Relativistic Gauge Field Equations \dotfill 44}
     \item[] \emph{Non-Relativistic Energie Functional \dotfill 45}
     \end{itemize}
   \end{itemize}
   \item[V] \textbf{Ortho- and Para-Positronium \dotfill 48}
     \begin{itemize}
     \item[1.] \emph{Conventional Multiplet Structure \dotfill 49}
     \item[2.] \emph{Ortho/Para Dichotomy in RST \dotfill 52}
     \item[3.] \emph{Positronium Eigenvalue Problem \dotfill 58}
     \end{itemize}
 \newpage
   \item[VI] \textbf{Energy Difference of Ortho- and Para-States \dotfill 66}
     \begin{itemize}
     \item[1.] \emph{Para-Positronium \dotfill 67}
        \begin{itemize}
        \item[] \emph{Electrostatic Approximation \dotfill 67}
        \item[] \emph{Spherically Symmetric Approximation\dotfill 71}
        \item[] \emph{Non-Relativistic Approximation \dotfill 75}
        \item[] \emph{Non-Relativistic Para-Spectrum \dotfill 78}
        \end{itemize}
     \item[2.] \emph{Ortho-Positronium \dotfill 86}
        \begin{itemize}
        \item[] \emph{Eigenvalue Problem for the Ortho-States \dotfill 86}
        \item[] \emph{Vanishing Angular Momentum $j_z=0$ \dotfill 87}
        \item[] \emph{Ortho-States with $j_z=-1$ \dotfill 90}
        \item[] \emph{Energy Functional for the Ortho-States \dotfill 95}
        \item[] \emph{Anisotropic and Magnetic Effects \dotfill 99}
        \item[] \emph{Non-Relativistic Energy Functional \dotfill 102}
    \end{itemize}
   \end{itemize}
   \end{itemize}
   \vspace{2ex}
   \noindent
   Appendix A:\\ 
   \phantom{Appe}\textbf{Manifest Gauge Invariance of the Energy Functional $\tETT$}\dotfill \textbf{106}\\[1ex]
   Appendix B:\\
     \phantom{Appe}\textbf{Variational Deduction of Non-Relativistic Eigenvalue Equations}
     \dotfill \textbf{108}\\[1ex]
   Appendix C:\\
     \phantom{App}\textbf{Variational Deduction of the Gauge Field Equations} \dotfill \textbf{112}\\[1ex]
   Appendix D\\
     \phantom{Appe}\textbf{Electric Poisson Identity} \dotfill \textbf{116}\\[1ex]
   Appendix E:\\
     \phantom{App}\textbf{Angular Part of the Ortho-Wave Amplitudes $\bMRpm,\bMSpm$} \dotfill \textbf{119}\\[1ex]
   Appendix F:\\
     \phantom{Appe}\textbf{Kinetic Energy ${}^{[b]}\tilde{T}_{\mathrm{kin}}$ of the
       Ortho-States } \dotfill \textbf{124}
     
   \newpage
\noindent
   Figure 1:\\
      \phantom{Figu}\textbf{Azimuthal Para-Current\ \ ${}^{(p)}k_\phi$} \dotfill \textbf{128}\\[1ex]
\noindent
   Figure 2:\\
      \phantom{Figu}\textbf{Non-Relativistic Para-Spectrum} \dotfill \textbf{129}\\[1ex]
\noindent
   Figure 3:\\
      \phantom{Figu}\textbf{Interaction Energy} { \ $\mathbf{\ERee=\tMMee} c^2$ } \dotfill \textbf{130}\\[1ex]
\noindent
   Figure 4a:\\
      \phantom{Figu}\textbf{Energy Curves}\ \ $\mathbf{\EET(\nu)}$ \dotfill \textbf{131}\\[1ex]
\noindent
   Figure 4b:\\
      \phantom{Figu}\textbf{Non-Relativistic Groundstate Energy}\dotfill \textbf{132}\\[1ex]
\noindent
   Figure 5:\\
      \phantom{Figu}\textbf{Angular Factors}\ \ $\mathbf{\bbko(\vartheta)}$ \textbf{for Ortho-Positronium}\dotfill \textbf{133}\\[1ex]
\noindent
   Figure 6:\\
      \phantom{Figu}\textbf{Azimuthal Ortho-Current}\ \ $\mathbf{\bbkphi}$ \dotfill \textbf{134}\\[4ex]

\noindent
\textbf{References  \dotfill 135} \\[4ex]
\textbf{Complete List of RST papers  \dotfill 137}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> macros.tex <==
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\vns}{\boldsymbol{\vec{\nabla}'}}
\newcommand{\ds}{\displaystyle}
\newcommand{\scr}{\scriptstyle}
\newcommand{\sscr}{\scriptstyle}
\newcommand{\e}{\operatorname{e}}
\newcommand{\mustbe}{\stackrel{!}{=}}
\newcommand{\rt}{(r,\vartheta)}
\newcommand{\rts}{(r',\vartheta')}


\newcommand{\sdot}{\,{\scriptscriptstyle{}^{\bullet}}\,}
\newcommand{\A}{\mathcal{A}}
\newcommand{\de}{\delta_{\textrm{e}}}
\newcommand{\ap}{{}^{(a)}\varphi_{\pm}(\vec{r})}
\newcommand{\app}{{}^{(a)}\varphi_{+}(\vec{r})}
\newcommand{\apm}{{}^{(a)}\varphi_{-}(\vec{r})}
\newcommand{\appm}{{}^{(a)}\varphi_{\pm}(\vec{r})}
\newcommand{\sappm}{{}^{(a)}\varphi\,'_{\pm}(\vec{r})}

\newcommand{\apmd}{{}^{(a)}\!\varphi_{\pm}^{\dagger}(\vec{r})}

\newcommand{\amd}{{}^{(a)}\!\varphi_{-}^{\dagger}(\vec{r})}
\newcommand{\apd}{{}^{(a)}\varphi_{+}^{\dagger}(\vec{r})}

\newcommand{\vp}[2]{ {}^{(#1)}\!\varphi_{#2} }
\newcommand{\dvp}[2]{{}^{(#1)}\!\varphi^\dagger_{#2} }

\newcommand{\ivpmp}{{}^{(1)}\varphi_{\mp}(\vec{r})}
\newcommand{\ivppm}{{}^{(1)}\varphi_{\pm}(\vec{r})}
\newcommand{\iivpmp}{{}^{(2)}\varphi_{\mp}(\vec{r})}
\newcommand{\iivppm}{{}^{(2)}\varphi_{\pm}(\vec{r})}
\newcommand{\iiivpmp}{{}^{(3)}\varphi_{\mp}(\vec{r})}
\newcommand{\iiivppm}{{}^{(3)}\varphi_{\pm}(\vec{r})}
\newcommand{\ipp}{{}^{(1)}\varphi_{+}(\vec{r})}
\newcommand{\ipm}{{}^{(1)}\varphi_{-}(\vec{r})}

\newcommand{\iipp}{{}^{(2)}\varphi_{+}(\vec{r})}
\newcommand{\iipm}{{}^{(2)}\varphi_{-}(\vec{r})}

\newcommand{\iiipp}{{}^{(3)}\varphi_{+}(\vec{r})}
\newcommand{\iiipm}{{}^{(3)}\varphi_{-}(\vec{r})}

\newcommand{\sPh}{{\stackrel{*}{\Phi}}(\vec{r}_1,\vec{r}_2)}
\newcommand{\sph}{{\stackrel{*}{\varphi}}}
\newcommand{\sphi}{{\stackrel{*}{\varphi}_1}(\vec{r}_1)}
\newcommand{\sphii}{{\stackrel{*}{\varphi}_2}(\vec{r}_2)}
\newcommand{\sphis}{{\stackrel{*}{\varphi}_1}(\vec{r}\,')}
\newcommand{\sphiis}{{\stackrel{*}{\varphi}_2}(\vec{r}\,')}

\newcommand{\hH}[1]{\hat{\mathcal{H}}_{\textrm{(#1)}}\,}
\newcommand{\shH}[1]{\hat{\mathcal{H}}\,'_{\textrm{(#1)}}\,}
\newcommand{\hh}[1]{\hat{\mathfrak{h}}_{\textrm{(#1)}}\,}
\newcommand{\shh}[1]{\hat{\mathfrak{h}}\,'_{\textrm{(#1)}}\,}
\newcommand{\hR}[1]{\hat{R}_{\textrm{(#1)}}\,}
\newcommand{\shr}[1]{\hat{r}\,'_{\textrm{(#1)}}\,}
\newcommand{\shR}[1]{\hat{R}\,'_{\textrm{(#1)}}\,}
\newcommand{\hr}[1]{\hat{r}_{\textrm{(#1)}}\,}

\newcommand{\aRpm}{{}^{(a)\!}\tilde{R}_\pm}
\newcommand{\aRp} {{}^{(a)\!}\tilde{R}_+{}}
\newcommand{\aRm}{{}^{(a)\!}\tilde{R}_-{}}
\newcommand{\iRp}{{}^{(1)\!}\tilde{R}_+{}}
\newcommand{\iRm}{{}^{(1)\!}\tilde{R}_-{}}
\newcommand{\iiRp}{{}^{(2)\!}\tilde{R}_+{}}
\newcommand{\iiRm}{{}^{(2)\!}\tilde{R}_-{}}
\newcommand{\ntR}{{}^{\{0\}}\!\tilde{R}}
\newcommand{\aSpm}{{}^{(a)\!}\tilde{S}_\pm}
\newcommand{\aSp}{{}^{(a)\!}\tilde{S}_+{}}
\newcommand{\aSm}{{}^{(a)\!}\tilde{S}_-{}}
\newcommand{\iSp}{{}^{(1)\!}\tilde{S}_+{}}
\newcommand{\iSm}{{}^{(1)\!}\tilde{S}_-{}}
\newcommand{\iiSp}{{}^{(2)\!}\tilde{S}_+{}}
\newcommand{\iiSm}{{}^{(2)\!}\tilde{S}_-{}}

\newcommand{\vSm}[1] { {}^{\textrm{(m)}}\!\vec{S}_{\textrm{#1}} }

\newcommand{\ikn}{{}^{(1)}\!k_0(\vec{r})}
\newcommand{\ikp}{{}^{(1)}\!k_\phi(\vec{r})}
\newcommand{\iikp}{{}^{(2)}\!k_\phi(\vec{r})}

\newcommand{\iikn}{{}^{(2)}\!k_0(\vec{r})}
\newcommand{\ikns}{{}^{(1)}\!k_0(\vec{r}\,')}
\newcommand{\iikns}{{}^{(2)}\!k_0(\vec{r}\,')}

\newcommand{\itkn}{{}^{(1)}\!\tilde{k}_0}
\newcommand{\iitkn}{{}^{(2)}\!\tilde{k}_0}

\newcommand{\itkp}{{}^{(1)}\!\tilde{k}_\phi}
\newcommand{\iitkp}{{}^{(2)}\!\tilde{k}_\phi}
\newcommand{\ijn}{{}^{(1)}\!j_0}
\newcommand{\iijn}{{}^{(2)}\!j_0}
\newcommand{\iiijn}{{}^{(3)}\!j_0}

\newcommand{\jj}[2]{ {}^{(#1)} {j^#2} }

\newcommand{\ajn}{{}^{(a)}\!j_0(\vec{r})}
\newcommand{\akn}{{}^{(a)}\!k_0\left(\vec{r}\right)}
\newcommand{\sakn}{{}^{(a)}\!k_0\left(\vec{r}\,'\right)}
\newcommand{\btkn}{{}^{(b)}\!\tilde{k}_0\left(r\right)}
\newcommand{\bkn}{{}^{(b)}\!k_0\left(\vec{r}\right)}
\newcommand{\bknn}{{}^{(b)}\!k_0\left(r\right)}
\newcommand{\btknn}{{}^{(b)}\!\tilde{k}_0\left(r\right)}
\newcommand{\aki}{{}^{(a)}\!k_1(\vec{r})}
\newcommand{\akp}{{}^{(a)}\!k_\phi(\vec{r})}
\newcommand{\akv}{\vec{k}_a(\vec{r})}

\newcommand{\aA}{{}^{(a)}\!A}
\newcommand{\vAa}{\vec{A}_a(\vec{r}}
\newcommand{\aAr}{{}^{(a)}\!A_0}
\newcommand{\aAe}{{}^{[a]}\!A_0}
\newcommand{\aAn}{{}^{(a)}\!A_0(\vec{r})}
\newcommand{\pAn}{{}^{(\textrm{p})}\!A_0(\vec{r})}
%\newcommand{\ppAn}{{}^{[\textrm{p}]}\!A_0(r)}
\newcommand{\ppAn}{{}^{[\textrm{p}]}\!A_0}
\newcommand{\nF}{{}^{\{0\}}\!F}
\newcommand{\nAn}{{}^{\{0\}}\!A_0}
\newcommand{\ppF}{{}^{[\textrm{p}]}\!F(r)}
\newcommand{\ppFn}{{}^{[\textrm{p}]}\!F(0)}

\newcommand{\iA}{{}^{(1)}\!\!A}
\newcommand{\iiA}{{}^{(2)}\!\!A}
\newcommand{\iiiA}{{}^{(3)}\!\!A}

\newcommand{\iAn}{{}^{(1)}\!\!A_0}
\newcommand{\iiAn}{{}^{(2)}\!\! A_0 }
\newcommand{\iiiAn}{{}^{(3)}\!\! A_0 }
\newcommand{\fAn}{{}^{(1/2)}\!\! A_0 }

\newcommand{\IA}{{}^{\textrm{(I)}}\!\!A}
\newcommand{\IIA}{{}^{\textrm{(II)}}\!\!A}
\newcommand{\IIIA}{{}^{\textrm{(III)}}\!\!A}
\newcommand{\AI}{A_{\textrm{I}}}
\newcommand{\AII}{A_{\textrm{II}}}
\newcommand{\AIII}{A_{\textrm{III}}}
\newcommand{\vAI}{\vec{A}_{\textrm{I}}}
\newcommand{\vAII}{\vec{A}_{\textrm{II}}}
\newcommand{\vAIII}{\vec{A}_{\textrm{III}}}
\newcommand{\AM}{\mathfrak{A}_{\textrm{M}}}
\newcommand{\An}{\mathfrak{A}_0}

\newcommand{\aVHS}{{}^{(a)}V_{\textrm{HS}}(\vec{r})}
\newcommand{\iVHS}{{}^{(1)}V_{\textrm{HS}}(\vec{r})}
\newcommand{\iiVHS}{{}^{(2)}V_{\textrm{HS}}(\vec{r})}

\newcommand{\onp}{\omega_0^\textrm{(+)}}
\newcommand{\onm}{\omega_0^\textrm{(-)}}
\newcommand{\oip}{\omega_1^\textrm{(+)}}
\newcommand{\oim}{\omega_1^\textrm{(-)}}
\newcommand{\onpm}{\omega_0^{(\pm)}}
\newcommand{\oipm}{\omega_1^{(\pm)}}

\renewcommand{\L}{\mathcal{L}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\as}{\alpha_{\textrm{s}}\,}
\newcommand{\aB}{a_{\textrm{B}}\,}
\newcommand{\aM}{a_{\textrm{M}}\,}
\newcommand{\ab}{a_{\textrm{b}}\,}
\newcommand{\Bstar}{\overset{*}{B}{} }
\newcommand{\vXstar}{\overset{*}{\vec{X}}}
\newcommand{\vYstar}{\overset{*}{\vec{Y}}}
\newcommand{\vBstar}{\overset{*}{\vec{B}}}
\newcommand{\Gstar}{\overset{*}{G}}
\newcommand{\gstar}{\overset{*}{g}}
\newcommand{\hstar}{\overset{*}{h}}
\newcommand{\vhstar}{\overset{*}{\vec{h}}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\GG}{\textnormal I \! \Gamma}
%\newcommand{\GG}{\mathbbm{\Gamma}}
\newcommand{\vfE}{\vec{\mathfrak{E}}}
\newcommand{\vfH}{\vec{\mathfrak{H}}}
\newcommand{\vfA}{\vec{\mathfrak{A}}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\FM}{F_{\textrm{M}}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\LRST}{\mathcal{L}_{\textrm{RST}}}
\newcommand{\LD}{\mathcal{L}_{\textrm{D}}}
\newcommand{\LG}{\mathcal{L}_{\textrm{G}}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\T}{\mathcal{T}}
\newcommand{\Mpe}{M_\textrm{p/e}\,}
\newcommand{\Mp}{M_\textrm{p}\,}
\newcommand{\Mee}{M^\textrm{(e)}}
\newcommand{\Me}{M_\textrm{e}\,}
\newcommand{\MT}{M_\textrm{T}}
\newcommand{\tMT}{\tilde{M}_\textrm{T}}
\newcommand{\MM}[1]{M_{[#1]}}
\newcommand{\Mei}{M_\textrm{I}^\textrm{(e)}}
\newcommand{\Meii}{M_\textrm{II}^\textrm{(e)}}
\newcommand{\Meiii}{M_\textrm{I/II}^\textrm{(e)}}
\newcommand{\Mmi}{M_\textrm{I}^\textrm{(m)}}
\newcommand{\Mmii}{M_\textrm{II}^\textrm{(m)}}
\newcommand{\Mmiii}{M_\textrm{I/II}^\textrm{(m)}}
\newcommand{\TT}{{}^{(\textrm{T})}T}
\newcommand{\DT}{{}^{(\textrm{D})}T}
\newcommand{\GT}{{}^{(\textrm{G})}T}
\newcommand{\hER}{\hat{E}_\textrm{R}}

\newcommand{\eER}{E_\textrm{R}^\textrm{(e)}}
\newcommand{\mER}{E_\textrm{R}^\textrm{(m)}}
\newcommand{\hEC}{E_\textrm{C}^\textrm{(h)}}
\newcommand{\gEC}{E_\textrm{C}^\textrm{(g)}}

\newcommand{\vH}[1]{\vec{H}_{\textrm{#1}}}

\newcommand{\EP}[1]{ E_{\textrm{P}(#1) }   }
\newcommand{\heER}{\hat{E}_\textrm{R}^\textrm{(e)}}
\newcommand{\hmER}{\hat{E}_\textrm{R}^\textrm{(m)}}
\newcommand{\ED}{{E_{\textrm{D}}}}
\newcommand{\EG}{E_{\textrm{G}}}
\newcommand{\Ec}{E_{\textrm{conv}}}
\newcommand{\cEc}{{\cal E}_{\textrm{conv}}}
\newcommand{\ET}{E_{\textrm{T}}}
\newcommand{\ETT}{E_{\textrm{[T]}}}
\newcommand{\tETT}{\tilde{E}_{\textrm{[T]}}}
\newcommand{\tbbETT}{\tilde{\mathbb{E}}_{\textrm{[T]}}}
\newcommand{\bbEIV}{\mathbb{E}^{\textrm{(IV)}}_{\textrm{[T]}}}
\newcommand{\Eiv}{E_\textrm{[T]}^{\textrm{(IV)}}}
\newcommand{\Epot}{ {\cal E}_{\textrm{pot}} }
\newcommand{\tET}{\tilde{E}_\textrm{T}}
\newcommand{\tETi}{\tilde{E}_\textrm{T}^{(|)}}
\newcommand{\tETii}{\tilde{E}_\textrm{T}^{(||)}}
\newcommand{\tEnT}{ {\tilde{E}^{(0)}_\textrm{T}} }
\newcommand{\tEnTmin}{ {\tilde{E}^{(0)}_\textrm{T,min}} }
\newcommand{\ETiii}{E_\textrm{T}^{(|||)}}
\newcommand{\Ekin}{{E_\textrm{kin}}}
\newcommand{\cEk}{{\cal{E}_\textrm{kin}}}
\newcommand{\ES}{{E_{\textrm{S}}}}
\newcommand{\EW}{{E_\textrm{W}}}
\newcommand{\HS}{H_{\textrm{S}}}
\newcommand{\hHin}{\hat{H}_{\textrm{in}}}
\newcommand{\hHS}{\hat{H}_{\textrm{S}}}
\newcommand{\WRST}{W_{\textrm{RST}}}
\newcommand{\WS}{W_{\textrm{S}}}
\newcommand{\lG}{{\lambda_\textrm{G}}}
\newcommand{\lGe}{ {\lambda_\textrm{G}^{(\textrm{e})}}\!}
\newcommand{\lGh}{ {\lambda_\textrm{G}^{(\textrm{h})}}\!}
\newcommand{\lGg}{ {\lambda_\textrm{G}^{(\textrm{g})}}\!}
\newcommand{\lGm}{  {\lambda_\textrm{G}^{(\textrm{m})}}\!\!}
\newcommand{\lGma}{  {\lambda_{\textrm{G}(a)}^{(\textrm{m})}}\!\!}
\newcommand{\lGem}{ {\lambda_\textrm{G}^{(\textrm{e/m})}}}
\newcommand{\lGema}{ {\lambda_{\textrm{G}(a)}^{(\textrm{e/m})}}}
\newcommand{\lD}{{\lambda_\textrm{D}}}
\newcommand{\lS}{{\lambda_\textrm{S}}}
\newcommand{\lpa}{\lambda_{\textrm{p}(a)}}
\newcommand{\NDa}{N_{\textrm{D}(a)}}
\newcommand{\np}{{n_\textrm{p}}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\NND}{\mathbb{N}_\textrm{D}}
\newcommand{\NNG}{\mathbb{N}_\textrm{G}}
\newcommand{\NNDa}{\mathbb{N}_{\textrm{D}(a)}}
\newcommand{\ND}{{N_\textrm{D}}}
\renewcommand{\NG}{{N_\textrm{G}}}
\newcommand{\NDn}{{N_\textrm{D}^\textrm{(0)}}}
\newcommand{\NGn}{{N_\textrm{G}^\textrm{(0)}}}
\newcommand{\NGe}{{N_\textrm{G}^\textrm{(e)}}}
\newcommand{\NNGe}{{\mathbb{N}_\textrm{G}^\textrm{(e)}}}
\newcommand{\NGh}{{N_\textrm{G}^\textrm{(h)}}}
\newcommand{\NNGh}{{\mathbb{N}_\textrm{G}^\textrm{(h)}}}
\newcommand{\NGg}{{N_\textrm{G}^\textrm{(g)}}}
\newcommand{\NNGg}{{\mathbb{N}_\textrm{G}^\textrm{(g)}}}
\newcommand{\nG}{{n_\textrm{G}}}
\newcommand{\snG}{{\tilde{n}_\textrm{G}}}
\newcommand{\nGe}{{n_\textrm{G}^\textrm{(e)}}}
\newcommand{\snGe}{{\tilde{}n_\textrm{G}^\textrm{(e)}}}
\newcommand{\nGh}{{n_\textrm{G}^\textrm{(h)}}}
\newcommand{\snGh}{{\tilde{n}_\textrm{G}^\textrm{(h)}}}
\newcommand{\nGg}{{n_\textrm{G}^\textrm{(g)}}}
\newcommand{\snGg}{{\tilde{n}_\textrm{G}^\textrm{(g)}}}
\newcommand{\NGm}{{N_\textrm{G}^\textrm{(m)}}}
\newcommand{\NGem}{{N_\textrm{G}^\textrm{(e,m)}}}
\newcommand{\nGm}{{n_\textrm{G}^\textrm{(m)}}}
\newcommand{\nGem}{{n_\textrm{G}^\textrm{(e,m)}}}
\newcommand{\LDk}{{\LD^{(\mathrm{kin})}}}
\newcommand{\LDe}{{\LD^{(\mathrm{e})}}}
\newcommand{\LDm}{{\LD^{(\mathrm{m})}}}
\newcommand{\LDM}{{\LD^{(\mathrm{M})}}}
\newcommand{\Tkin}{{T_\textrm{kin}}}
\newcommand{\oWD}{{\overset{\circ}{W}\!}_\textrm{D}}
\newcommand{\oWG}{{\overset{\circ}{W}\!}_\textrm{G}}
\newcommand{\oWRST}{{\overset{\circ}{W}\!}_\textrm{RST}}
\newcommand{\oWRSTe}{{\overset{\circ}{W}}{}^{\textrm{(e)}}_\textrm{RST}}
\renewcommand{\S}{\mathcal{S}}
\newcommand{\Ph}{\Phi(\vec{r}_1,\vec{r}_2)}
\newcommand{\VN}{V_\NN}
\newcommand{\TN}{T_\NN}
\newcommand{\cTN}{\mathcal{T}_\NN}
\newcommand{\PN}{P_\NN}
\newcommand{\pN}{(p_0,p_1,\ldots p_\NN) }
\newcommand{\cVN}{\mathcal{V}_\NN}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\covnab}{{\boldsymbol{\vec{\nabla}{}'}}}
\newcommand{\covlap}{\boldsymbol{\Delta\!'}}
\newcommand{\dkmat}{\delta^\dagger_\textrm{mat}}
\newcommand{\tEET}{\tilde{\mathbb{E}}_\textrm{[T]}}
\newcommand{\vmSe}{{}^\textrm{(m)}\vec{S}_1}
\newcommand{\vmSz}{{}^\textrm{(m)}\vec{S}_2}
\newcommand{\vmSd}{{}^\textrm{(m)}\vec{S}_3}
\newcommand{\EPa}{E_{{\rm P}(a)}}
\newcommand{\ERe}{{E_\textrm{R}^\textrm{(e)}}}
\newcommand{\ERm}{{E_\textrm{R}^\textrm{(m)}}}
\newcommand{\ECh}{{E_\textrm{C}^\textrm{(h)}}}
\newcommand{\ECg}{{E_\textrm{C}^\textrm{(g)}}}
%\newcommand{\NDa}{N_{{\rm D}(a)}}
\newcommand{\lDa}{\lambda_{{\rm D}(a)}}
\newcommand{\lPa}{\lambda_{{\rm P}(a)}}
\newcommand{\lPe}{\lambda_{{\rm P}(1)}}
\newcommand{\lPz}{\lambda_{{\rm P}(2)}}
\newcommand{\lPd}{\lambda_{{\rm P}(3)}}
\newcommand{\MMg}{{\mathbb{M}^\textrm{(g)}}}
\newcommand{\MMgconv}{{\mathbb{M}_\textrm{conv}^\textrm{(g)}}}
\newcommand{\MMgpol}{{\mathbb{M}_\textrm{pol}^\textrm{(g)}}}
%\newcommand{\NNDa}{\NN_{{\rm D}(a)}}
%\newcommand{\NNGe}{{\NN_\textrm{G}^\textrm{(e)}}}
%\newcommand{\NNGh}{{\NN_\textrm{G}^\textrm{(h)}}}
%\newcommand{\NNGg}{{\NN_\textrm{G}^\textrm{(g)}}}
\newcommand{\aphip}{{}^{(a)}\varphi_+}
\newcommand{\aphim}{{}^{(a)}\varphi_-}
%\newcommand{\appm}{{}^{(a)}\varphi_{\pm}}
\newcommand{\epp}{{}^{(1)}\varphi_{+}}
\newcommand{\epm}{{}^{(1)}\varphi_{-}}
\newcommand{\zpp}{{}^{(2)}\varphi_{+}}
\newcommand{\zpm}{{}^{(2)}\varphi_{-}}
\newcommand{\zppm}{{}^{(2)}\varphi_{\pm}}
\newcommand{\dpp}{{}^{(3)}\varphi_{+}}
\newcommand{\dpm}{{}^{(3)}\varphi_{-}}
\newcommand{\bb}{\mathbbm{b}}
\newcommand{\Ih}{\mathbbm{h}}
\newcommand{\zz}{\mathbbm{z}}
\newcommand{\ZZ}{\mathbb{Z}}
%\newcommand{\hstar}{\overset{*}h}
\newcommand{\vbb}{\vec{\bb}}
\newcommand{\vIh}{\vec{\Ih}}
\newcommand{\vzz}{\vec{\zz}}
\newcommand{\vZZ}{\vec{\ZZ}}
\newcommand{\vbbstar}{\overset{*}{\vec{\bb}}}
\newcommand{\vIhstar}{\overset{*}{\vec{\Ih}}}
\newcommand{\vzzstar}{\overset{*}{\vec{\zz}}}
\newcommand{\vZZstar}{\overset{*}{\vec{\ZZ}}}
\newcommand{\adn}{{}^{(a)}\!\delta_0}
\newcommand{\idn}{{}^{(1)}\!\delta_0}
\newcommand{\iidn}{{}^{(2)}\!\delta_0}
\newcommand{\iiidn}{{}^{(3)}\!\delta_0}
\newcommand{\Ij}{{}^{\textrm{(I)}}\!j}
\newcommand{\IIj}{{}^{\textrm{(II)}}\!j}
\newcommand{\IIIj}{{}^{\textrm{(III)}}\!j}
\renewcommand{\ij}{{}^{(1)}\!j}
\newcommand{\iij}{{}^{(2)}\!j}
\newcommand{\iiij}{{}^{(3)}\!j}
\newcommand{\adup}{{}^{(a)}\!\delta_\uparrow}
\newcommand{\idup}{{}^{(1)}\!\delta_\uparrow}
\newcommand{\iidup}{{}^{(2)}\!\delta_\uparrow}
\newcommand{\iiidup}{{}^{(3)}\!\delta_\uparrow}
\newcommand{\Bdo}{{}^{(B)}\!\delta_0}
\newcommand{\Bdup}{{}^{(B)}\!\delta_\uparrow}
\newcommand{\Tkina}{{T_{\textrm{kin}(a)}}}
\newcommand{\Tkine}{{T_{\textrm{kin}(1)}}}
\newcommand{\Tkinz}{{T_{\textrm{kin}(2)}}}
\newcommand{\Tkind}{{T_{\textrm{kin}(3)}}}
\newcommand{\tNGm}{{\tilde{N}_\textrm{G}^\textrm{(m)}}}
\newcommand{\hNGm}{{\hat{N}_\textrm{G}^\textrm{(m)}}}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main_minenergy"
%%% End: 

